A Case study of light pollution in France after the change in legislation

France issued a decree to restrict and prohibit mainly outdoor lighting effective from January 1st, 2019. Effectiveness of this legislation has been evaluated in this study using GIS data which was first used in \cite{2020MNRAS.493.1204A} (so called astroGIS database - \url{astrogis.org}). A subset of Artificial Light layer of astroGIS database has been adapted for years between January 2012 and December 2019. During 2019, radiance of $1.9 \times 10^{9}$ W cm$^{-2}$ sr$^{-1}$ has been released into space. Annual light pollution in France decreased by 6\% after the enactment of artificial light legislation. France continue to have potential Dark Sky Park locations for example cities like Indre, Lot, Nievre and Creuse having the lowest light pollution values. A strong correlation between population and light pollution ($R\simeq 0.83$) has been observed. A similar but a weak correlation can also be observed for GDP ($R\simeq 0.28$). However, it is still too early to justify whether the improvements observed in the dataset are due to the enactment of the legislation or not.

==> old/respons_to_reviewer_I.tex <==
Shortly after our manuscript was published in ArXiv (arXiv: 2006.04440), a researcher responded with a feedback about airglow correction on VIIRS detector after 2017, and directed us to the article DOI:10.3390/s20113287. We've studied this feedback and finally updated all our dataset using the masks stated in the related articles and website. Therefore, the article's mainframe is almost changed from the previous submission. We've updated all related sections accordingly.

Answers to reviewer's comments & questions:

[REVIEWER]
The authors use satellite data to analyze artificial lights at night over France aiming to assess light pollution conditions after the legislation change. Although the light pollution topic is well within the scope of Astrophysics and Space Science, the manuscript in its present form is rather suitable for a non-astronomical journal. The authors should pay more attention to potential consequences for astronomy.

[OUR RESPONSE]
We completely reshaped the article by implementing reviewer's suggestions. Here are the key changes we've done:
- Light pollution of the observatories in France added and discussed.
- The earlier title was implying mostly a work on effect of legislation. We've changed it to a more science oriented title.
- Now, the introduction reflects more on astronomical impact of light pollution.
----------

[REVIEWER]
[1] page 1, line 45-46: A strong correlation between population and light pollution is indicated. However, the value of R=0.83 is not so high to say the correlation is strong. I would like to bring to the authors attention the criticism of population-based models published only recently in MNRAS Letters (Volume 496, Issue 1, July 2020, Pages L138-L141).

[OUR RESPONSE]
When we use recalibrated dataset and working with luminous flux units, lumens (see section 3), we found good demographic correlations with light pollution [population (R^2= 0.85) and GDP (R^2= 0.84)]. The article suggested by the reviewer doesn't contain all cities, however ours contain all. We have now a clear view of outliers for both demographic values and therefore, when they are excluded the correlations clearly becomes high.
----------

[REVIEWER]
[2] Introduction is more than 30% of the paper, and, there is no clear correlation between what has beed said in the Intro and what is brought in the result-section.

[OUR RESPONSE]
The reviewer was right; the introduction is reorganized.
---------- 

[REVIEWER]
[3] page 3, line 8-9, left column: A list of cities is long for France (for instance, there are 434 major cities in France with population 20,000+, https://simple.wikipedia.org/wiki/List_of_cities_in_France).

[OUR RESPONSE]
France is divided into 13 regions and 96 departments (excluding overseas ones). They are further divided into smaller groupings where we think that they are beyond our scope of the dataset because demographic data becomes unreliable for these minor groupings (see https://www.wikiwand.com/simple/France#Divisions).

Since we exclude data below the sensor limit of 3 nW cm^{-2} sr^{-1} (2013JGRD..11812705L) we have to stay on stable grouping of departments (aka. cities). On the other hand most of these 434 regions are expected to stay below the sensor's limit.
---------- 

[REVIEWER]
[4] page 3, line 17-18, right column: existence of new legislation does not necessarily means the lighting technology conversion is started or even completed instantaneously. I understand the author's motivation for this study, but I don't believe anything really changed in 2018/2019 in France. Some examples: LED conversion started in Vienna in 2017 and it will take several years to complete this process (the partial goal for 2020 is to complete modernization of 50000 lamps: https://www.wien.gv.at/verkehr/strassen/einrichtungen/beleuchtung/led-tausch/auftaktveranstaltung.html). The same process has lasted 3 years in Tucson (JQSRT 212, 10-23, 2018). For sure the legislation change cannot result in an immediate streetlight conversion over the whole country.

[OUR RESPONSE]
After the complete rewrite and using new calibrated dataset, reviewer's point become more obvious. Therefore, we've updated related points stated through out the article. The 8 years of "change" now looks more like "remaining constant" except for years after 2017.
---------- 

[REVIEWER]
[5] page 3, line 22-23, right column: what are the criteria used to select 4 highest and 4 lowest light polluting cities? Normally, the larger city, the higher light flux upwards. But this doesn't mean a large city should be classified as highly light polluting source. A modern lighting technology installed in a large city can result in lowered value of lumens-per-head or lumens-per-area compared to to what can be observed in a smaller city in which lighting conversion did not started. How the authors distinguished cities with high and low light pollution levels? What's about lighting inventory?

[OUR RESPONSE]
After the rewrite, again, city-specific changes disappeared and therefore we presented "all cities" to reflect both steady variation of AL and re-calibration of the sensor in 2017. However, AL levels of the cities show almost four discrete groups: over-luminous, luminous, typical, under luminous.

Note that, since we intend to stay on the astronomical level the lightning inventory was not in our scope in this work.
---------- 

[REVIEWER]
[6] page 3, line 39-40, right column: the light emission from total surface area of France is discussed, but the units provided is W/cm2/sr, i.e. it is still a value per square cm.

[OUR RESPONSE]
The unit confusion is cleared through out the manuscript.
---------- 

[REVIEWER]
[7] page 3, lines 45-49, right column: A good statistics of radiance data need to be available for each city to draw such conclusion as in the paper. What is the number of radiance-data taken for each single city? How can you guarantee a decreaser 27 cities is real? Were the data taken under same conditions? (season, atmospheric turbidity, satellite viewing angle,…).

[OUR RESPONSE]
The reviewer's point on "need more radiance data" is also our conclusion, too. As we stated in previous points, conclusion of "decrease in AL" is totally abandoned. 

Note also that, after airglow correction, AL variation is too small to be considered as a significant change. In addition to this, many masking can be used in daily measurements: moonlight, lightning, proximity to the pole, seasonal coverage, etc. Therefore, when these are excluded, a time-independent AL value could be produced.
---------- 

[REVIEWER]
[8] page 3, lines 50-53, right column: The emission function of a city can show seasonal and spectral behaviors (see Fig. 2 and the text at page 7714 in PNAS (7712-7717, April 16, 2019, vol. 116, no. 16). Any conclusions drawn for a city need to be done carefully taking into account spectral response of a sensor, viewing (zenith) angle, season, ground albedo and type of vegetation for a city. This can result in a large uncertainty in percent change the authors have evaluated, especially if the above factors are unknown.

[OUR RESPONSE]
The reviewer was right. We dropped this completely. However, we believe that these effects tend to converge to a minimum level in the long-term.
---------- 

[REVIEWER]
[9] page 3, lines 54-57, right column: Were winter and summer data treated separately when making the statistical analysis? It seems the authors tend to interpret 6% decrease as a result of legislation change. However, the proof for such a claim is necessary.

[OUR RESPONSE]
Due to the nature of satellite, France is not covered through out annually (DOI:10.1080/01431161.2017.1342050). Therefore, depending on the orientation of the satellite (especially spring to summer months: ~ may-august) dataset was varying monthly. Therefore, monthly averages are collected only if all cities have a data, making a uniform data structure for all cities within the scope of the time span.

---------- 

[END]

==> old/respons_to_reviewer_II.tex <==
[REVIEWER]
The authors responded to all my concerns, while some other do not materialize since the authors have removed criticized parts of the article.
The article is now improved, however, a short paragraph on a potential uncertainty of satellite data should be included as suggested in my previous comment #8.
It should be explained in the paragraph that the emission function of a city can show seasonal and spectral behaviors (PNAS, 7712-7717, April 16, 2019, vol. 116, no. 16) that can impact the signals detected by satellite.
The emission function can depend on the wavelength meaning that there is some error tolerance we need to accept when processing a broadband signal at the satellite.

[OUR RESPONSE]
We've overlooked reviewer's comment #8 and forgot to mention CEF effect. Now this has been added as the last paragraph of Data Analysis section.

Through out the reviewing process, the reviewer gave us valuable and positive comments. Therefore we've acknowledged this at the end of the paper.
